Exploring the Long Short-Term Dependencies to Infer Shot Influence in Badminton Matches

Identifying significant shots in a rally is important for evaluating players' performance in badminton matches. While there are several studies that have quantified player performance in other sports, analyzing badminton data is remained untouched. In this paper, we introduce a badminton language to fully describe the process of the shot and propose a deep learning model composed of a novel short-term extractor and a long-term encoder for capturing a shot-by-shot sequence in a badminton rally by framing the problem as predicting a rally result. Our model incorporates an attention mechanism to enable the transparency of the action sequence to the rally result, which is essential for badminton experts to gain interpretable predictions. Experimental evaluation based on a real-world dataset demonstrates that our proposed model outperforms the strong baselines. The source code is publicly available at https://github.com/yao0510/Shot-Influence.

==> tables/experiment-dataset.tex <==
\begin{tabular}{lr}
    \toprule
    Statistics                      & Value\\
    \midrule
    \# of shots                     & 15742\\
    \# of rallies (sequences)       & 1409\\
    \# of sets                      & 46\\
    \# of matches                   & 19\\
    Average length of rallies       & $\sim11$\\
    Ratio of wins to losses (rally) & 680 : 729\\
    Ratio of wins to losses (set)  & 18 : 28\\
    Ratio of wins to losses (match) & 7 : 12\\
    \bottomrule
\end{tabular}

==> tables/experiment-reason-true-proportion.tex <==
\begin{tabular}{lr}
    \toprule
    End reason        & Accuracy and detailed counts\\
    \midrule
    Misjudge          & 0.000 (0/5)\\
    In                & 0.700 (35/50)\\
    Out               & 0.815 (53/65)\\
    Touch net         & 0.878 (43/49)\\
    Not pass over net & 0.962 (25/26)\\
    \bottomrule
\end{tabular}
